Safe Road-Crossing by Autonomous Wheelchairs: a Novel Dataset and its Experimental Evaluation

Safe road-crossing by self-driving vehicles is a crucial problem to address in smart-cities. In this paper, we introduce a multi-sensor fusion approach to support road-crossing decisions in a system composed by an autonomous wheelchair and a flying drone featuring a robust sensory system made of diverse and redundant components. To that aim, we designed an analytical danger function based on explainable physical conditions evaluated by single sensors, including those using machine learning and artificial vision. As a proof-of-concept, we provide an experimental evaluation in a laboratory environment, showing the advantages of using multiple sensors, which can improve decision accuracy and effectively support safety assessment. We made the dataset available to the scientific community for further experimentation. The work has been developed in the context of an European project named REXASI-PRO, which aims to develop trustworthy artificial intelligence for social navigation of people with reduced mobility.

==> 01_introduction.tex <==
\section{Introduction}\label{sec:intro}
Self-driving vehicles have attracted a huge interest in the intelligent transportation systems industry. Those vehicles are equipped with advanced sensors providing data to computing systems running \emph{Artificial Intelligence} (AI) algorithms that enable them to operate and navigate without human intervention. They offer the promise of increased safety and performance. These vehicles rely on several technologies, including LiDARs, radars, cameras, and sophisticated software to perceive their surroundings, make decisions, and control their movements \cite{autonomous_vehicles}. However, all those technological innovations based on AI and \emph{Machine Learning} (ML) come with big challenges in terms of trustworthiness, due to limited transparency and failures possibly having fatal consequences in safety-critical systems \cite{9979717}. This is also the case of \emph{Autonomous Wheelchairs} (AWs) that are meant to support motion-impaired persons in safe door-to-door navigation.

There have been several efforts to improve the technology of powered wheelchairs since their first appearance during the 19th century~\cite{yukselir2012brains}. Modern AWs can be very complex including sophisticated components, such as autonomous navigation system, and aim to accommodate several disabilities by means of multi-modal interfaces. Safety assessment and certifications of AWs are paramount aspects to address \cite{tas23}. In fact, in presence of components based on AI, together with specific regulations such as ``ISO 7176-14:2022 Wheelchairs'',\footnote{\url{https://www.iso.org/standard/72408.html}} other requirements and guidelines must be considered such as the ones included in the EU Artificial Intelligence Act.\footnote{\url{https://artificialintelligenceact.eu}}

The work described in this paper has been developed within the European project REXASI-PRO (REliable \& eXplAinable Swarm Intelligence for People with Reduced mObility),\footnote{\href{https://rexasi-pro.spindoxlabs.com/}{https://rexasi-pro.spindoxlabs.com/}} which addresses indoor and outdoor use cases to demonstrate trustworthy social navigation of autonomous wheelchairs together with flying drones in real-world environments. Drones are used to provide a view of the environment from different perspectives and thus collect additional data %that can be possibly used 
to scan and map the surrounding environment. 

In this paper, we deal with a road-crossing scenario using multiple sensors and with no support of traffic lights. We adopt multi-sensor fusion for run-time risk-based decision support. To this aim, we use laboratory wheeled robots, equipped with artificial vision and distance sensors, as mock-up models of actual AWs and drones, for which we perform run-time safety evaluation using an analytical danger function based on physical considerations.

The main original contributions of this paper can be summarized as follows:
\begin{itemize}
    \item We provide a novel reference scenario for road-crossing by AWs as well as hints and details about laboratory experimentation and performance evaluation.
    \item We share with the scientific community a specific dataset 
    %that we have generated using
    with data recorded from multiple sensors that can be used for further experimentation and performance evaluation.
    \item We introduce an approach for road-crossing decision making based on an analytical and hence explainable danger function highlighting the importance of multi-sensor obstacle detection. 
    \item As a proof-of-concept, we report the results of a preliminary experimental evaluation demonstrating the advantages of using diverse redundant sensors, which can support safety certification when used in combination with probabilistic safety models.
\end{itemize}

The remaining of this paper is structured as follows. Sec.~\ref{sec:lit} provides an overview of the related literature. Sec.~\ref{sec: road-crossing} introduces the reference road-crossing scenario. Sec.~\ref{sec:df} describes the design of the danger function. Sec.~\ref{sec:data_gen } addresses dataset generation in the laboratory environment. Sec.~\ref{sec:exp} reports the results of the experimental evaluation. Finally, Sec.~\ref{sec:conclusion} provides conclusions and hints about future developments.

\section{Related works}\label{sec:lit}
%Data fusion techniques combine data from multiple sensors, and related information from associated databases, to achieve improved accuracies and more specific inferences than could be achieved by the use of a single sensor alone \cite{hall}.
%\subsection{Systems for safe for road-crossing}

Pedestrians and wheelchair users are among the most vulnerable group type in transport systems and traffic environments \cite{Pedestrian,Obstacles_wheel,statistics2019analysis}. Being road-crossing especially dangerous, it is one of the most investigated situation in terms of pedestrian–vehicle conflict to prevent accidents \cite{ELHAMDANI2020102856}.
%Solutions include installation of infrastructures that help pedestrians at intersection and cross way. 
%
In \cite{Crosswalk}, authors propose a crosswalk safety warning system where both pedestrian and vehicle behaviour is detected and evaluated by multiple sensors; warning alerts are communicated to both parts through lights integrated in the cross path infrastructure. In \cite{10010764}, a smart traffic light control system equipped with a camera is used to manage pedestrian crossing considering the traffic condition and type of pedestrian; crossing is improved for the elderly or people with disabilities without worsening traffic.
In \cite{9043590}, authors propose a vision-based approach to generate safety messages in real-time using video streams from roadside traffic cameras; the messages can be used by connected autonomous vehicles and smart phones equipped with pedestrian safety applications.
Given the costs of such approaches, virtual reality is a useful tool to simulate smart pedestrian crossing \cite{guo2023smart}, particularly if designed for wheelchair users \cite{Co-Designing-VR}.

%Devices on board vehicles can also help reduce the risk of road accidents. In \cite{5936735}, an active pedestrian safety system based on stereo vision is design and tested. Sensing, situation analysis and decision making are combined to control the vehicle and avoid collision.


Although those solutions represent an aid for wheelchair users, they need a specific and possibly expensive infrastructure.
%they need a specific solution independent by cities infrastructures and therefore possibly incorporated in AWs. 
%, . It is therefore necessary for the AW to have danger analysis and evaluation system on board.
%Questions surrounding the problem of risk assessment from PWUs point of view are under-explored especially in the context of road-crossing.
In \cite{Wheel_video}, ML is used to elaborate the videos of on-board cameras and to support AW decisions. A similar approach is applied in \cite{INDRA}, where a convolutional neural network is suitably designed to evaluate the risk of road-crossing on Indian roads. Compared to our approach, those works are based on single ML technologies lacking sufficient redundancy, diversity and transparency, and as such less suitable for safety assessment.

%All those works do not Compared to those works, we focus on the design of an explainable danger function using the outputs of reundant   do not overlap with the scope and objectives of our paper.
%This approach does not enhance safety due to the lack of robustness and transparency. 
%In fact, a support system based uniquely on one typology of sensor may be subject to failure if this stops working properly \cite{laprie2008dependability} and ML methods present issues related to explainability \cite{arrieta:hal-02381211}

%To the best of our knowledge, the work described in this paper is the first one addressing robust run-time risk assessment for AWs using multiple sensors in the context of road-crossing. A novel function is designed starting from assumptions on what factors are important for PWUs to achieve safe road-crossing. Then, consideration are done to obtain the danger assessment related to the kinematics characterising the road-crossing problem. Finally as a proof-of-concept, we report the results of a preliminary experimental evaluation where obstacle detection is carried out with multiple sensors in order to enhance robustness.
%Furthermore Ml methods used for object detection within the autonomous driving model face the problem of high demand for processing large amounts of data, which places high performance requirements on the algorithms.


\begin{figure}
  \centering
  \begin{minipage}{1\linewidth}
    \centering
    \subfloat{\includegraphics[width=.32\linewidth]{images/scene1.png}}
    \subfloat{\includegraphics[width=.32\linewidth]{images/scene2.png}}
    \subfloat{\includegraphics[width=.32\linewidth]{images/scene3.png}}

    \caption*{(a)}
  \end{minipage}\quad
  \begin{minipage}{1\linewidth}
    \centering
    \subfloat{\includegraphics[width=.32\linewidth]{images/scene1.png}}
    \subfloat{\includegraphics[width=.32\linewidth]{images/scene2b.png}}
    \subfloat{\includegraphics[width=.32\linewidth]{images/scene4.png}}
    \caption*{(b)}
  \end{minipage}

\caption{Road-crossing scenario: drone and AW cooperate to support safe decisions, e.g., when a car surpasses the crossing location (a), or when a car stops before the crossing location (b).}
\label{fig:syntet_scen}
\end{figure}




\section{Reference scenario for safe road-crossing}\label{sec: road-crossing}
%In this section are discussed the design for the road-crossing scenario that we consider and the considerations on what are the main aspects that help to evaluate a danger situation in such scenario. These are used afterwards in Sec.~\ref{sec:df}.


%\subsection{Safe road-crossing}\label{subsec: safe_road_cros}
When crossing a road, especially where there are no traffic lights, humans consider a variety of factors to ensure both safety and convenience. Primarily, they assess the flow of traffic, considering variables like the speed and quantity of vehicles. They also account for the presence of road-crossings, traffic signals, and zebra crossings, as these demarcate safe areas for traversing. The distance to the nearest crossing point and the estimated time required to reach it are taken into consideration, as are potential traffic delays that might offer a safer crossing opportunity. Additionally, individuals evaluate their own physical capabilities for quick crossing and gauge the visibility of oncoming vehicles. Factors such as weather conditions, the presence of children or elderly, and the accessibility of nearby sidewalks also affect the decision. Ultimately, the act of crossing a road involves a multifaceted interplay of these considerations, striking a balance between personal safety and the need to reach the destination efficiently.

In our analysis, we assume that pedestrians account for distance, speed and acceleration (\cite{PAPIC2020105586} and \cite{acceleration}) as pivotal cues in their assessment of approaching vehicles before determining whether it is safe to cross the road. These factors provide vital insights into how rapidly a vehicle is closing in and whether adequate time exists for a safe crossing.

\paragraph*{Distance.} The distance of an approaching vehicle is a central indicator on which pedestrians heavily rely. Distance perception is related to the personal experience of each single pedestrian. For example it might be affected by the physical condition of the pedestrian, the weather condition or other elements that can affect the time required to perform crossing. 

\paragraph*{Speed.} People gauge speed through visual cues, such as changes in the vehicle's apparent size and the interval it takes for the vehicle to traverse a specific distance between reference points on the road. A vehicle that is swiftly shortening the gap is generally perceived as moving at a higher speed, while one with a more gradual progression may be perceived as moving slower. 

\paragraph*{Acceleration.} Pedestrians also consider acceleration, denoting how swiftly an object alters its speed over time. Acceleration contributes to the decision-making process by signaling how quickly a vehicle may reach the pedestrian's location. Consequently, this can influence the choice to wait for the vehicle to pass before attempting to cross. 

%For instance, if a pedestrian notices a vehicle initially distant but accelerating rapidly, they might deduce that the vehicle could cover the distance to them in less time than initially estimated. This realisation could prompt them to delay crossing until the vehicle has passed, even if their initial perception of the distance suggests safety. Conversely, when pedestrians observe a nearby vehicle decelerating, they interpret this as a sign that the vehicle is preparing to halt, potentially allowing a safer crossing opportunity. %Deceleration implies that the vehicle will take longer to traverse the remaining distance to the pedestrian, affording more time for a secure road-crossing. This cue can alleviate some of the urgency pedestrians might feel when confronted with a fast-approaching vehicle. Nevertheless, pedestrians must remain cautious and factor in the broader traffic context, as a decelerating vehicle could also be adjusting its speed due to obstacles or impending turns, thereby altering its trajectory.

%Distance, speed and acceleration contribute to pedestrians' comprehension of how imminently a vehicle is approaching and whether an appropriate interval exists for road-crossing.
%These factors are considered in the next section to define our risk evaluation method.


%\subsection{Design of the road-crossing scenario} \label{subsec:Design_scenario}
\hfill \break
We apply a similar reasoning to the road-crossing scenario for AWs, where the system must take a safe road-crossing decision. Following the principles of redundancy and diversity, a safe decision must be based on multiple sensors using different technologies whose accuracy is affected by mostly independent factors \cite{Flammini2020}. This can be achieved, for instance, by combining cameras featuring artificial vision with LiDARs or other distance sensors. Additional information can be obtained by connecting the AW with drones or specific infrastructures \cite{9043590}, providing information from diverse sources or different perspectives. %These data can be used to assess the DF discussed in the previous section.

The road-crossing scenario we consider consists of an AW on the side of a one-way road aiming to reach the other side, a drone connected to the AW that provides further information and a vehicle approaching the specific section of the road. We assume that there are no traffic lights and the driver’s behaviour is not predictable; he/she might slow down to allow the crossing or move ahead, maintaining its motion. Hence, the AW must use its sensing capabilities to estimate the potential danger: the crossing is safe if the danger is estimated under a certain threshold. If the danger is too high, crossing is not recommended until the vehicle slows down or surpasses the crossing location. This is why it is important to design a danger function, as described in the next section. Fig.~\ref{fig:syntet_scen} provides a schematic representation of the scenario.



==> 02_methodology.tex <==
%\section{Risk Assessment????}

%\begin{itemize}
%    \item Multi-sensor approach 
%    \item DATA ELABORATION in synthesis 
%    \item 
%    \item fusion: at three possible levels
%\end{itemize}


%When dealing with dangerous situation as road crossing, autonomous systems have to ensure high level of safety. This is particularly important for those devices that deal with fragile subjects as AW.
%However, it is not enough for a system to be secure, it should be also trusted by the user, who otherwise would not be induced to use it.


%For this purpose we propose a risk-based decision support system that rely on a multi-sensors information fusion system. The use of sensors that differ by a software or a technological point of view should prevent vulnerabilities to become single points of failure \cite{laprie2008dependability}. Moreover, technology redundancy and diversity are good features to improve resilience against environmental disturbances and to increase robustness against malfunctions and, to some extent, to reduce the costs by using cheaper components.

%Several sensors located on the AW measure the distance between the wheelchair itself and possible approaching vehicles, from which speed and acceleration are calculated. The danger is evaluated by this three values through the Danger Function, properly designed for the crossing road context. If the danger exceed a certain threshold value then the system detects a dangerous situation and advises against the crossing. Each sensor provides a certain information which may or may not be correct depending on the status of the sensor or particular environmental conditions. Consequently an appropriate combination of this data is necessary.

%The next two subsections describe the Danger Function with the motivations which led to its particular design choice and how the sensor data combination is

%Usually dangerous situations during road crossing are evaluated in correspondence with the pedestrian passage or traffic light, where the driver is expected to slow down after a certain reaction time. Therefore this behaviour can be included in the assessment of possible dangerous situations. Unfortunately, these considerations are invalid in all those cases where there are no infrastructures to aid the crossing. Or it might be consider too optimistic that they are always applicable. 



==> 03_case_study.tex <==
%This involves the following three agents:
%\begin{itemize}
    %\item \textbf{Autonomous wheelchair}: An autonomous wheelchair is standing still and uses multiple, i.e., camera, LiDARs and distance sensors to monitor the road where vehicles might come from.
    %\item \textbf{Drone}: A flying drone stays on the other side of the road and uses a camera to provide a different perspective of the road.
    %\item \textbf{Car}: A vehicle, such as a car, approaches the section of the road that the AW aims to cross. Its motion is unpredictable.
%\end{itemize}

%Therefore, the autonomous wheelchair should be equipped with multiple sensors. Therefore, we assume a multi agent and multi modal sensing system approach. Sensors outputs are combined to provide a common decision
%Principles leading the design of hardware and software components of sensor systems are:
%\paragraph*{Redundancy}
%Redundancy refers to including extra or duplicated elements within a system to enhance its fault-tolerance. 
%The usage of diverse redundant detectors in safety-critical monitoring applications allows to tackle two challenges:
%\begin{itemize}
%    \item Reduce reliability-growth costs, which can be kept linear instead of exponential;
%    \item Reach higher security standards when even the most expensive single technology can be demonstrated to comply with required levels .
%\end{itemize}
%\paragraph*{Diversity}
%Diversity means using sensors based on different technologies and/or sensing from different perspectives (e.g., from the wheelchair and from the drone). Diverse sensors are less prone to common causes of failures such as obstructions or environmental disturbances. % affected by different to capture a wide range of information, enhancing the robot's perception and adaptability to its environment. Diversity is crucial when external conditions make a type of sensor less reliable (e.g. cameras in rain conditions). 
%\section{System sensor design}
%The experimental scenario must reproduce principles used to design the real reference system. Most importantly redundancy and diversity.
%In the real system redundancy is guaranteed from different sensors used to look at the surrounding environment. The presence of a camera on the wheelchair and one on the drone is an example of redundancy. 
%Therefore, we equipped both the agent representing the wheelchair and the one representing the drone with cameras featuring artificial vision using motion tracking. From a hardware standpoint in the experiment, we equipped both cameras and range sensors on the agents to guarantee hardware diversity. It is also possible to equip different software on the agent to obtain software diversity.

%\subsection{Sensor System Design}
%Redundancy and Diversity
%Evaluate Reliability
%\subsection{Preprocessing}


%\subsection{Assumptions on the reference scenario}
%The setting of this thesis work is the plausible scenario of a road-crossing. 



%\paragraph*{Assumptions and limitations}
%We limited the initial scope of our experiment to a one-way road, where the incoming vehicles can only come from one side.
%We also discarded a scenario where the obstacle goes past the wheelchair aiming to cross and then comes back to pass again on the same section of the road. 

%This makes it possible to point sensors in the direction of the incoming vehicle and not on the other side of the road.


%The use of an assistive device such as a drone equipped with a camera allows to diversify the information used by the risk assessment process by exploiting  a second point of view. This is crucial when the AW encounter occlusions or obstructions that hinder sensor detection.

\section{Dataset generation} \label{sec:data_gen }
In this section, we provide the specification of the laboratory environment --- including all the equipment and hardware components --- and describe the procedure of data collection, data pre-processing and data elaboration. In the experiments, we target a similar scenario as described in Sec.~\ref{sec: road-crossing}. 
%Because the real system hardware components (i.e., depth cameras, LiDARs, and the AW itself) are expensive, for this proof-of-concept, low cost components are adopted instead, in a 
We adopt a simplified experimental setup, where three ground robots equipped with vision and distance sensors represent the AW, drone and vehicle, as depicted in Fig.~\ref{fig:Scenes}. In our lab, we can access ground truth poses from a very accurate motion tracking system.

\subsection{Laboratory environment}
The experiments have been performed in %a $10 \times 10 \times 2$ $m^3$ room of 
the \emph{IDSIA Autonomous Robotics Laboratory}.\footnote{\href{https://idsia-robotics.github.io}{https://idsia-robotics.github.io}}

\paragraph{Robots.}
For our experiments we use three wheeled omni-directional robots: each one is a RoboMaster EP (RM), a commercial education platform from DJI,\footnote{\href{https://www.dji.com/ch/robomaster-ep}{https://www.dji.com/ch/robomaster-ep}} whose specifications are summarized in Tab.~\ref{tab:Robomaster_spec}.
%
%
% and the main technologies used are \emph{RoboMaster} and \emph{OptiTrack}.
%
% \emph{RoboMaster} EP (RM) is a commercial education platform from DJI~\cite{rm}. For the experiments, we use three omnidirectional ground wheeled robots, whose main features are in Tab.~\ref{tab:Robomaster_spec}. 
Each RM is customised for its role as ``car'', ``AW'', or ``drone''.
% One robot is provided with a gimbal and the others with a robotic arm.  
\begin{description}
\item[RM$_\mathrm{c}$] simulates the vehicle and does not require additional sensors, as we are interested just on its movement.
\item[RM$_{\mathrm{w}}$] represents the AW and is equipped with a camera and four infrared range sensors. Given their narrow \emph{Field Of View} (FOV) (see Tab.~\ref{tab:Robomaster_spec}), range sensors are located on the RM so that their outputs can be combined to obtain information for a larger FOV. The RM$_{\mathrm{w}}$ and its sensors are shown in Fig.~\ref{fig:Scenes}b. Conservatively, we consider the minimum distance reading returned by the four range sensors, which from now on we refer to as the single sensor \emph{Range Sensors Unit} (RSU).
\item[RM$_{\mathrm{d}}$] acts as the drone and has a camera positioned on top of the robotic arm.
\end{description}
% One of the RM with the robotic arm is used to simulate the vehicle (RM$_\mathrm{c}$) and does not require additional devices since we are interested just on its movement.
% The one with the gimbal works as the AW (RM$_{\mathrm{AW}}$) and is equipped with a camera and four infrared range sensors. Given their narrow FOV (see Tab.~\ref{tab:Range_spec}), range sensors are located on the RM so that their outputs can be combined to obtain information for a larger FOV. 
% *** Franca? *** In practice, following an over-cautious approach, we take the minimum distance value returned by the four sensors. The last one, the drone (RM$_{\mathrm{D}}$), has a camera positioned on top of the robotic arm. The specifications of the cameras and infrared range sensors installed on the RMs are provided in Tab.~\ref{tab:Camera_spec} and Tab.~\ref{tab:Range_spec}.

\begin{table}[htp]
\centering
\begin{tabular}{lll}
%Weight &  3.3 kg \\
\hline
\multirow{3}{*}{Chassis} & size & \qtyproduct{32 x 24 x 27}{cm}\\
& maximal speed & \SI{3.5}{m/s}\\  
& maximal angular speed& \SI[per-mode=symbol]{600}{\degree\per\second}\\
\hline
\multirow{3}{*}{Camera}  & FOV & \ang{120} \\
% & sensor & CMOS 1/4 inch \\
& video resolution & 1280 x 720 \\
& video fps & \SI{30}{\Hz} \\
\hline
\multirow{3}{*}{Range sensors} & maximal range & \SI{10}{m} \\
& FOV & \ang{20} \\
& accuracy & \SI{5}{\percent}\\
\hline
\end{tabular}
\caption{Technical specifications of RoboMaster EP.}
\label{tab:Robomaster_spec}
\end{table}


%EP (for educational pack) Core replaces the gimbal with a parallel mechanism arm and a gripper. The camera is mounted on the arm. It has a metal extension to the plastic chassis to mount various other parts, such as ToF sensors and IO adapters.



%\paragraph*{RM sensors}



%\paragraph*{Technical Specifications}
%Technical specifications of cameras installed on the RoboMaster:

%\paragraph*{ROS2}


% \begin{table}
%     \centering
%     \begin{tabular}{|ll|}
%         \hline
%         FOV & $ 120 ^\circ$ \\
%         Maximum resolution & $2560\times1440$ \\
%         Maximum video resolution & FHD: $1.080/30$ fps \\
%         & HD: $720/30$ fps\\
%         Max video bitrate & 16 Mbps \\
%         Sensor & CMOS $1/4"$\\
%         \hline
%     \end{tabular}
%     \caption{Technical specifications of cameras.}
%     \label{tab:Camera_spec}
% \end{table}



%\paragraph*{Sensors}
%\paragraph*{Infrared Range Sensor}
%\paragraph*{Technical Specifications}

%The infrared range (or distance) sensors installed on the RoboMaster simulating the AW are based on the time of flight (TOF) principle, i.e., the sensors emit modulated near-infrared light, which is reflected when it strikes an object. Each sensor then computes the distance to the object by calculating the time difference or phase difference between light emission and reflection. 
%\paragraph*{Features}
%The sensor emits a conical light with an angle of $20^\circ$. The relationship between the spot (D) and the distance (Dist) is calculated as follows: 

%\begin{equation}\label{eq:distance}
%\begin{aligned}
%D = 2 \times \text{Dist} \times \tan(10)
%\end{aligned}
%\end{equation}


% \begin{table}
%     \centering
%     \begin{tabular}{|ll|}
%         \hline
%         Detection Range & $0.1 - 10 m$ \\
%         FOV & $20^\circ$ \\
%         Accuracy & $5\%$ \\
%         \hline
%     \end{tabular}
%     \caption{Technical specifications of the infrared distance sensor.}
%     \label{tab:Range_spec}
% \end{table}

%\paragraph*{OptiTrack v2.3}
\paragraph{Motion Tracker.}
The lab used for the experiments is equipped with an OptiTrack motion tracker\footnote{\href{https://docs.optitrack.com/v/v2.3}{https://docs.optitrack.com/v/v2.3}} composed of eighteen infrared cameras covering an area of \qtyproduct{6x6x2}{\meter} to track the pose of the three robots at \SI{30}{Hz} with sub-millimetre accuracy. %The motion tracker provides ground truth for our experiments.  
%Thanks to the high accuracy and quality, we can use the data generated by this system as the ground truth for our experiments.  

%It is widely used in various industries, including animation, virtual reality, sports analysis, robotics, and research. OptiTrack uses a network of high-speed cameras to track the movements of markers or objects with exceptional accuracy and precision. The captured data can be used to animate characters, analyze human or animal movements, control virtual objects, or provide real-time feedback for live applications. OptiTrack's reliable and versatile tracking capabilities make it a popular choice for professionals and enthusiasts seeking high-quality motion capture solutions.
%\paragraph*{OptiTrack and ROS2}
%The machine connected to the OptiTrack system must be running ROS2 and be connected to the machine making the recordings via Local Area Network. It will run a node for the OptiTrack and create a topic for each object the tracker is following. The node making the recording must be subscribed to all the topics from the Optitrack node.

%\paragraph*{Robot Operating System (ROS2)}
%The Robot Operating System (ROS) \cite{ROS} is a set of software libraries and tools for building robot applications designed to build robot applications. It provides a flexible and modular framework for developing, controlling, and simulating robotic systems. With ROS2, it is possible to easily integrate various sensors, actuators, and algorithms. The concept behind ROS 2 is to break complex systems down into many modular nodes and use topics to allow them to interact.

%We interface with the several RMs the Robot Operating System (ROS) \cite{ROS}. To control robots and record data, a ROS2 driver for the DJI Robomaster family of robots (EP and S1) based on the official Python client library used\footnote{\href{https://github.com/jeguzzi/robomaster\_ros}{https://github.com/jeguzzi/robomaster\_ros}} is used.



%\paragraph*{Nodes}
%Any program that has access to ROS functionalities and ROS communications is a ROS Node. Each node in ROS should be responsible for a single, modular purpose. The concept at the base of ROS functioning is to have multiple nodes running simultaneously and interacting. Each node can send and receive data from other nodes via topics, services, actions, or parameters.
%\paragraph*{Topics}
%Topics act as a bus for nodes to exchange messages. A node can publish on multiple topics and can be subscribed to multiple topics. Many nodes can publish on a single topic and many nodes can be subscribed to a topic.
%\paragraph*{Rosbag}
%Rosbag is a file format and toolset in the Robot Operating System (ROS) that allows users to record, store, and playback data from ROS topics. It serves as a powerful tool for logging and capturing data generated during robotic experiments, simulations, or real-world deployments. ROS bag files can store various data types, including sensor readings, robot states, and other messages. Researchers and developers can replay the recorded data later for analysis, debugging, or testing, making it a valuable asset for robotics applications and research.

%\paragraph*{RVIZ2}
%RVIZ is a ROS graphical interface that allows to visualize a lot of information, using plugins for many kinds of available topics. RVIZ2 is simply a port of RVIZ into ROS 2. We used RVIZ2 to visualize data retrieved from topics produced from the OptiTrack ROS2 node. 

==> 04_Danger_Function.tex <==



\section{Design of the danger function}\label{sec:df}
In this section, we address the problem of assessing the risk associated with road-crossing based on what discussed in the previous section. The road-crossing scenario includes an AW attempting to cross the road and an oncoming obstacle (e.g., a car). As shown in Fig.~\ref{fig:raod_crossing}, the two bodies are assumed to have orthogonal motions, with the pedestrian crossing the road from one side to the other while the vehicle proceeds along the driveway.

In our approach, the risk evaluation is based on a continuous function $g$, called \emph{Danger Function} (DF). The function is intended to reflect a kinematic analysis of the road-crossing scenario in a particular moment $t$. Accordingly, the value of the DF reflects the danger level associated with the kinematic configuration of the system at a specific moment. For decision-making, we summarise the assessments provided by the DF $g$ by tagging them as potentially dangerous if the corresponding DF values exceed a given threshold $g^*$.

\begin{figure}[htp!]
    \centering
    \includegraphics[width=9cm]{images/geometry_cross_scen.png}
    \caption{Kinematics involved in the design of the danger function.}
    \label{fig:raod_crossing}
\end{figure}

To derive the DF, we assume that the AW can proceed with uniform linear motion and the obstacle approaches it with a uniformly accelerated motion. Both assumptions are often unrealistic, but might reflect an over-cautious modelling providing a safer evaluation: in real scenarios, in case of danger, the vehicle would likely slow down and the AW would likely accelerate.

We consequently model the road-crossing scenario as follows. Assuming the AW crossing the road to move on the x-axis and starting the crossing from position $x=0$ with constant speed $v_{\mathit{w}}$, we have:
\begin{equation}\label{eq:wheelchair}
x_{\mathit{w}}(t) = v_{\mathit{w}} \cdot t\,.
\end{equation}
Similarly, assuming the obstacle, i.e., the car, moving on the y-axis with constant acceleration $a_c$ and initial speed $v_c$:
\begin{equation}\label{eq:obstacle}
y_c(t) = v_c \cdot t + \frac{a_c}{2} \cdot t^2\,.
\end{equation}
From Eq.~\eqref{eq:wheelchair}, we can compute the time $t_{\mathrm{cross}}$ required by the AW to cross a road of width $l$, i.e., $t_{\mathrm{cross}}:=l/v_{\mathit{w}}$. During the interval of time $[0,t_{\mathrm{cross}}]$, the obstacle should be far enough to not impact with the AW, i.e., if $d_c$ is the distance of the obstacle: 
\begin{equation}\label{eq:s_min}
d_c > v_c \cdot t_{\mathrm{cross}} + \frac{a_c}{2} \cdot t_{\mathrm{cross}}^2\,,
\end{equation}
and hence:
\begin{equation}\label{eq:constraint}
\frac{\frac{l}{v_{\mathit{w}}}\cdot v_c + \frac{l^2}{2 \cdot v_{\mathit{w}}^2} \cdot a_c}{d_c}<1\,.
\end{equation}

We can regard the constraint in Eq.~\eqref{eq:constraint} as a safety condition for a kinematics-based DF with threshold one. As expected, the danger increases for higher values of speed and acceleration of the car, while decreasing for increasing distances. Assessing all the parameters of such a DF might be critical when coping with different road-crossing scenarios. For this reason, we heuristically define a DF $g$, with similar relations with $d_c$, $v_c$ and $a_c$ as in Eq.~\eqref{eq:constraint}, whose parameters might be reasonably assessed for a generic scenario.

Regarding the inverse dependence with respect to $d_c$, we assume that close objects are significantly more dangerous than distant objects, even if they are moving at lower speed. Consequently, to enhance the impact of the distance on the function in specific situations where the two bodies are close, a logarithm smoothing is applied to  $d_c$. Moreover, a small threshold $\epsilon$ is also added to always obtain finite values.
Concerning the linear combination of speed and acceleration in the numerator of the left-hand side of Eq.~\eqref{eq:constraint}, we perform linear transformations with threshold on both $v_c$ and $a_c$, and denote the output of these transformations as $\hat{v}_c$ and $\hat{a}_c$ and use a coefficient $k$ to evaluate the relative contribution of the speed with respect to the acceleration.
%Overall we obtain: 
Therefore the DF is described as:
\begin{equation}\label{eq:complete}
g(d_c, v_c, a_c) := \frac{\hat{v}_c + k \cdot \hat{a}_c}{\log (d_c + \epsilon)}\,,
\end{equation}
where $k=0.1$ and $\epsilon=0.6$ are set following heuristics. The linear transformation of the speed is:
\begin{equation}\label{eq:speed_component}
\hat{v}_c :=
\begin{cases} 
0&\text{if }v_c \leq \underline{v}_c\,,\\
\frac{v_c-\underline{v}_c}{\overline{v}_c-\underline{v}_c}&\text{if }\underline{v}_c< v_c\leq \overline{v}_c\,,\\
1&\text{if }v_c > \overline{v}_c\,,\\
\end{cases}
\end{equation}
and, for the acceleration:
\begin{equation}\label{eq:acceleration_component}
\hat{a}_c:=
\begin{cases} 
-1&\text{if }a_c\leq -\overline{a}_c\\
\frac{a_c+\underline{a}_c}{\overline{a}_c-\underline{a}_c}&\text{if }-\overline{a}_c < a_c \leq -\underline{a}_c\\
0&\text{if }-\underline{a}_c<a_c\leq \underline{a}_c\\
\frac{a_c-\underline{a}}{\overline{a}_c-\underline{a}_c}&\text{if }\underline{a}_c < a_c  \leq \overline{a}_c\\
1 & \text{if }a_c > \overline{a}_c\,.\\
\end{cases}
\end{equation}
The above transformations are intended to prevent contributions to the DF by low speeds (i.e., $v_c\leq \underline{v}_c$) and low accelerations (i.e., $|a_c|\leq \underline{a}_c$), while also putting a normalised upper bound to the contributions of high speeds ($v_c \geq \overline{v}_c$) and accelerations ($|a_c| \geq \overline{a}_c$).
Fig.~\ref{fig:va} shows the choice of the threshold parameters $\underline{v}_c$, $\overline{v}_c$, $\underline{a}_c$, and $\overline{a}_c$, we considered for the experimental setup (Sec.~\ref{sec:exp}).

Fig.~\ref{fig:df_tracker} shows an example of the kinematics (for clarity, only distance and speed on the left) and the corresponding values of the DF (right). %More details are in Sec.~\ref{sec:exp}.




\begin{figure}[htp!]
\centering
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
axis lines=middle,
xmax=0.8,
xmin=-0.1,
ymin=0,
ymax=1.1,
xtick={0.05,0.65}, 
label style = {font=\large},
ticklabel style = {font=\large},
xticklabels={$\underline{v}_c=0.05$,$\overline{v}_c=0.65$},
ytick={0.0,1.0},    
yticklabels={$0$,$1$},
xlabel={$v$  ($\frac{m}{s}$)},
ylabel={$\hat{v}_c$}]
\draw[black,very thick] (0,0) -- (0.05,0);
\draw[black,very thick] (0.05,0) -- (0.65,1);
\draw[black,very thick] (0.65,1) -- (0.8,1);
\draw[dotted] (0.65,0) -- (0.65,1);
\end{axis}
\end{tikzpicture}
%
\phantom{aa}
%
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
axis lines=middle,
xmax=13,
xmin=-13,
ymin=-1.1,
ymax=1.1,
xlabel={$a_c$ ($\frac{m}{s^2}$)},
ylabel={$\hat{a}_c$},
ticklabel style = {font=\large},
label style = {font=\large},
xticklabels={$\underline{a}_c=1$, $\overline{a}_c=10$},
xtick={2.5,10},
ytick={-1,0,1}]
\draw[black,very thick] (-13,-1) -- (-10,-1);
\draw[black,very thick] (10,1) -- (13,1);
\draw[black,very thick] (-1,0) -- (1,0);
\draw[black,very thick] (-10,-1) -- (-1,0);
\draw[black,very thick] (10,1) -- (1,0);
\draw[dotted] (10,0) -- (10,1);
\draw[dotted] (-10,0) -- (-10,-1);
\end{axis}
\end{tikzpicture}
\caption{Linear transformations with threshold used for $v_c$ (left) and $a_c$ (right).}
\label{fig:va}
\end{figure}

\begin{figure}[htp!]  
\centering 
\begin{tikzpicture}[scale=0.7,baseline]
\pgfplotsset{xmin=0,xmax=5}
\begin{axis}[axis y line*=left,ymin=0, ymax=3, xlabel=$t$ (s),ylabel=distance $d$ (m)]
\addplot[thick,color=black,mark=none] table [smooth,x=timestamp,y=distance_tracker,col sep=comma]{all.csv};
\label{plot:distance}
\end{axis}
\begin{axis}[axis y line*=right,axis x line=none,ymin=0, ymax=0.6,ylabel=speed $v$ (m/s)]
\addlegendimage{/pgfplots/refstyle=plot:distance}\addlegendentry{distance}
\addplot[thick,dotted,color=black,mark=none] table[smooth,x=timestamp, y=speed_tracker, col sep=comma]{all.csv};
\addlegendentry{speed}
\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.7,baseline]
\pgfplotsset{xmin=0,xmax=5}
%\draw[fill=green,opacity=0.1]  (0,0) -- (6.85,0) -- (6.85,2.29) -- (0,2.29) -- cycle;
%\draw[fill=red,opacity=0.1]  (0,5.7) -- (6.85,5.7) -- (6.85,2.29) -- (0,2.29) -- cycle;
\begin{axis}[ytick={0.0,1.0,1.5},yticklabels={$0.0$,$g^*$,$1.5$},ymin=0, ymax=1.5,xlabel=$t$ (s),ylabel=danger level $g$]
\addplot[color=black,thick] table[mark=none,smooth,x=timestamp,y=danger_tracker,col sep=comma]{all.csv};
\draw[dotted,line width=0.25mm] (0,1) -- (10,1);
\end{axis}
\end{tikzpicture}
\caption{Distance, speed (left) and DF values (right) on the experiment in Sec.~\ref{sec:exp}.}\label{fig:df_tracker}
\end{figure}

==> 04_dataset.tex <==
\subsection{Data collection and preprocessing} \label{subsec:Data_prepr}
As in the scenario described in Sec.~\ref{sec: road-crossing}, RM$_{\mathrm{w}}$ and RM$_{\mathrm{d}}$ are motionless and oriented towards the approaching RM$_{\mathrm{c}}$, which is remotely controlled. 

\paragraph{Data collection.}
To control the robots and collect data from the motion tracker, we used the \emph{Robot Operating System} (ROS2~\cite{ROS}), executing a ROS2 driver for each robot.\footnote{\href{https://github.com/jeguzzi/robomaster\_ros}{https://github.com/jeguzzi/robomaster\_ros}}
%This method is a good solution for obtaining aligned data, that is paramount during data processing. 
% To control robots and record data, a ROS2 driver for the DJI RoboMaster family of robots (EP and S1) based on a Python client library\footnote{\href{https://github.com/jeguzzi/robomaster\_ros}{https://github.com/jeguzzi/robomaster\_ros}} is used. 
For each experimental run, we recorded data from the two cameras, the RSU and the motion tracker in bag files as detailed in Tab.~\ref{tab:Dataset_spec}. 


\begin{figure}[htp!]%
\centering
%{\includegraphics[trim={0 0 0 0},clip,width=5cm]{images/scene A.png} }%
\subfloat[]{\includegraphics[height=4.5cm]{images/sceneA.png}}
\hfill
\subfloat[]{\includegraphics[height=4.5cm]{images/RMsensors.png}}

\caption{(a) Example of setup for data collection: in red is the trajectory of RM$_{\mathrm{c}}$ and in blue the crossing path of RM$_{\mathrm{w}}$. (b) RM$_{\mathrm{w}}$ and its components.}
\label{fig:Scenes}%
\end{figure}



Overall, we recorded 15 runs for two different setups (the first one is depicted in Fig.~\ref{fig:Scenes}a), for which runs last approximately \SI{6}{s} and resp. \SI{9}{s}. In the second setup, the initial distance of the RM$_{\mathrm{c}}$ with respect to the RM$_{\mathrm{w}}$ is larger, allowing for more complex patterns in movement of the obstacle during experiments.



% \begin{table}[htp]
% \centering
% \begin{tabular}{lp{1cm}rp{1cm}rrr}
% \hline
% Source/Fusion Technique&&RMSE&&Accuracy&Recall&Precision\\
% \hline
% Range sensors&&0.582&&{\bf 0.92}&0.89&{\bf 0.99}\\
% AW camera&&0.948&&0.77&{\bf1.0}&0.59\\
% Drone camera&&1.923&&0.51&0.63&0.32\\
% \hline
% Distance fusion&&0.447&&{\bf 0.92}&0.91&0.95\\
% Danger fusion&&{\bf 0.361}&&0.83&0.78&0.96\\
% Voting fusion&&-&&0.67&0.50&0.38\\
% \hline
% \end{tabular}
% \caption{Evaluation of the quality of the different sensors and fusion techniques in terms of RMSE of the DF and precision, accuracy and recall of the decisions based on the DF and its threshold.}
% \label{tab:rmse}
% \end{table}

\begin{table}[htp]
\centering
\begin{tabular}{llll}
\hline
Name & Source & Type & Frequency \\
\hline
Poses of RM$_{\mathrm{w}}$, RM$_{\mathrm{d}}$ and RM$_{\mathrm{c}}$  & Motion Tracker& 2D poses & \SI{30}{Hz}\\
Video & RM$_\mathrm{w}$ & $1080\times720$ RGB images & \SI{30}{Hz} \\
Video & RM$_\mathrm{d}$  & $1080\times720$ RGB images & \SI{30}{Hz} \\
Range sensors & RM$_\mathrm{w}$ & 4 distances to nearest object   & \SI{10}{Hz} \\
\hline
\end{tabular}
\caption{Raw data recorded during the experiments.}
\label{tab:Dataset_spec}
\end{table}


\paragraph{Data pre-processing.}
Raw data from the bag files were processed to synchronise all streams. 
Relative distances between RM$_{\mathrm{w}}$ and RM$_{\mathrm{c}}$ were computed for ground truth poses and from RSU.
%
% In this regard, the relative distance between RM$_{\mathrm{w}}$ and RM$_{\mathrm{c}}$ is chosen as comparison quantity. Optitrack records are easily elaborated starting from the poses of RM$_{\mathrm{w}}$ and RM$_{\mathrm{c}}$. Removing a bias value due to the size of RM$_{\mathrm{w}}$, the range sensors raw data on RM$_{\mathrm{w}}$ already give the desired measure so their information is directly combined.
%
Raw data from cameras were split using OpenCV\footnote{\href{https://docs.opencv.org/4.x/index.html}{https://docs.opencv.org/4.x/index.html}} into frames. These were processed with \emph{You Only Look Once} (YOLO)\footnote{\href{https://github.com/ultralytics/yolov5}{https://github.com/ultralytics/yolov5}} \cite{redmon2016look}, a commonly used Machine Learning model, to detect RM$_{\mathrm{c}}$. RMs do not have a specific class in YOLO, but are consistently recognised as \emph{motorcycles}. YOLO was used to identify their bounding boxes in image space, from which we computed the distance using 
triangle similarity.\footnote{\href{https://pyimagesearch.com/2015/01/19/find-distance-camera-objectmarker-using-python-opencv/}{https://pyimagesearch.com/2015/01/19/find-distance-camera-objectmarker-using-python-opencv/}}
% Given an image of an object with an apparent width $P$, if the actual width of object is $W$ and the camera focal length is $F$, then the distance $D$ from the camera to the object is $D:=W \times F/P$.
%
% The distance from RM$_{\mathrm{c}}$ are obtained from the two cameras on RM$_{\mathrm{w}}$ and RM$_{\mathrm{d}}$ in this way. This two distance measures are almost identical as shown in the Fig.~\ref{fig:Scenes}, therefore the distance measure of the camera on RM$_{\mathrm{d}}$ is not further modified. 
%
Finally, the three distance measures from the sensors onboard, i.e. closed RSU and the two cameras, were smoothed, taking an average of the previous 2 (RSU) or 5 (cameras) samples . 

% Then the data are ready to be elaborated. 

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{images/triangle_similarity.png}
%    \caption{Triangle similarity. Source \cite{triangle_similarity}}
%    \label{fig:triangle}
%\end{figure}


%\paragraph*{Experimental Data Processing}
%Data from Optitrack represents the absolute positions of every agent at every time $t$. It is available at 30 Hz. Data from range sensors represents the distance between the wheelchair agent and the incoming obstacle at every time $t$ It is available at 10 Hz. Images from cameras on the wheelchair and the drone agents represent the point of view of the agent, it needs to be processed by applying Computer Vision algorithms. It is available at 30 Hz. 

%Data from Optitrack was only processed to get from absolute positions, relative distances, speeds, and accelerations.





%The data have been collected in a $10$ x $10$ m room equipped with a motion capture system (mocap), composed of 18 Optitrack PM13 cameras.

%The dataset is intended for use in multi-sensor and swarm configurations, thanks to multiple, redundant and diverse information sources recorded simultaneously during experiments.

%The setting of data collection is an approximation of the real road situation in which autonomous wheelchairs, with the task of helping patients with reduced mobility, and autonomous drones, will make road-crossing decisions. 

%\subsection{Data Collection}
%The available datasets for the task of safe road-crossing have limited sensor information sources and are not collected in a swarm configuration setup. The objective of data collection was to create a novel dataset, specifically tailored for the task of safe road-crossing in a swarm configuration. The swarm configuration allows us to place multiple robots in different positions in the room and obtain more diverse data. 

%To generate the dataset, we used 3 DJI Robomaster EP, i.e., wheeled ground robots. The robots are equipped with a camera, which provides a 120 degree field of view with a maximum resolution of 2560 × 1440, The camera is capable to record full-HD videos at 30 fps, for 1 robot is mounted on a gimbal and for the other robot it is mounted on a robotic arm. The robot equipped with a gimbal is additionally equipped with 4 range sensors, the gimbal is never moved by the teleoperator during the experiment. The camera from robot 3 has not been recorded. All the robots are fitted with omnidirectional wheels and have onboard a mocap target (i.e. relfective marker). Thanks to the markers applied, on all the robots, the mocap system can track their pose, resulting in a precise ground truth labeling information. These poses are recorded using the ROS framework , and synchronised with the video frames (streamed to a host computer via WiFi from the robots).

%We teleoperated robots during experiments via hoast computer using ROS. 
%All experiments feature data from 7 different data sources: the motion capture system, 2 RoboMaster cameras, 4 distance sensors installed on the RoboMaster simulating the AW.



\subsection{Data elaboration and sensor fusion} 
\label{subsec:DATA_elab}
Speed and acceleration measures were computed from the four distance measures obtained from the RSU, the two cameras and the tracker.
Then, danger was estimated for each sensor using the function described in Sec.~\ref{sec:df}. When the danger value exceeded the given threshold, a dangerous situation was detected and crossing was not recommended. An example of the results is shown in Fig.~\ref{fig:video}: three frames from the RM$_{\mathrm{w}}$ camera output are displayed with the corresponding DF value calculated by the tracker. A dot in green (resp. red) defines a safe (resp. dangerous) situation as a result of the threshold criterion.

Since three values can be obtained from the RSU and the two cameras, a fusion procedure is required. 
Raw data from sensors are already aligned, but have different sampling times. 
All measures were therefore resampled at 100 Hz before merging.
We considered three different fusion architectures. A straightforward fusion procedure consists of taking the average of the distances measured by the three sensors. We call this procedure \emph{distance fusion}. We call instead \emph{danger fusion} the fusion procedure where the average of the DFs computed by the distances measured by the three sensors is considered. Finally, \emph{voting fusion} was applied to the values obtained after the threshold operation on the DFs through a majority vote. All the data collected are available, together with the code used for processing and analysis, in a freely available repository.\footnote{\href{https://github.com/CarloGrigioni/safe_roadcrossing_aw}{https://github.com/CarloGrigioni/safe\textunderscore roadcrossing\textunderscore  aw}}.

\begin{figure}[h]
\centering
\subfloat{\includegraphics[width=.34\linewidth]{images/video1.png}}
\subfloat{\includegraphics[width=.34\linewidth]{images/video2.png}}
\subfloat{\includegraphics[width=.34\linewidth]{images/video3.png}}
\caption{Example of the results: RM$_{\mathrm{w}}$ camera frames number 6, 60 and 90 with corresponding DF calculated by ground truth (tracker) measures.}
\label{fig:video}
\end{figure}

%We expect the fusion of the distances measures to be the most performing one, since the data at that level contain the most information content before being further processed \cite{hall}.



%\paragraph{Sensor Fusion}
%Data from range sensors needed a preliminary fusion, due to the different orientations of the 4 sensors. The approach was to trust the value from the sensor measuring the shortest distance, which was the one with the best orientation to correctly sense the incoming obstacle.
%The overall fusion strategy consisted in weighting the contribution of each sensor based on two factors: the general confidence in that sensor, and the quality of readings just before time $t$.

%The possible approaches for sensor fusion are:
%\begin{itemize}
%    \item Weighted average
%    \item Weighted voting
%\end{itemize}

%Considering the 4 range sensors together the readings obtained are the most similar to the ones from OptiTrack we use as ground-truth, thus the most reliable. Given this information, we want to keep the contribution of the range sensors to the function after sensor fusion predominant.

%\subsection{Results}

\begin{figure}[htp!]  
\centering 
\begin{tikzpicture}[baseline]
\pgfplotsset{xmin=0.5,xmax=4.2}
\begin{axis}[
width=.5\textwidth,
height=.22\textheight,
legend style={at={(0.54,0.53)}},
axis y line*=left,ymin=0, ymax=2.5, xlabel=$t$ (s),
xtick={0.0,1.0,2.0,3.0,4.0},ylabel=distance $d$ (m)]
\addplot[thick,color=orange,mark=none] table [smooth,x=timestamp,y=distance_range,col sep=comma]{sensors.csv};
\addlegendentry{\tiny{range sensors}}
\addplot[thick,color=red,mark=none] table [smooth,x=timestamp,y=distance_wheelchair,col sep=comma]{sensors.csv};
\addlegendentry{\tiny{AW camera}}
\addplot[thick,color=blue,mark=none] table [smooth,x=timestamp,y=distance_drone,col sep=comma]{sensors.csv};
\addlegendentry{\tiny{drone camera}}
\addplot[thick,dotted,color=black,mark=none] table [smooth,x=timestamp,y=distance_tracker,col sep=comma]{sensors.csv};
\addlegendentry{\tiny{tracker}}
\end{axis}
\end{tikzpicture}
% \hfill
\begin{tikzpicture}[baseline]
\pgfplotsset{xmin=0.5,xmax=4.2}
\begin{axis}[
width=.5\textwidth,
height=.22\textheight,
legend style={at={(0.65,0.5)}},
axis y line*=left,ymin=0, ymax=2.5, xlabel=$t$ (s),
xtick={0.0,1.0,2.0,3.0,4.0}]
\addplot[very thick,color=black,mark=none] table [smooth,x=timestamp,y=distance_fusion,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{distance fusion}}
\addplot[thick,dotted,color=black,mark=none] table [smooth,x=timestamp,y=distance_tracker,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{tracker}}
\end{axis}
\end{tikzpicture}
\caption{Distance as recorded by the different sensors (left), by the ground truth (tracker)  and after the \emph{distance fusion} (right).}
\label{fig:distance_sensors}
\end{figure}

\section{Experimental evaluation}\label{sec:exp}
In this section, we present the results of the three fusion approaches described in Sec.~\ref{subsec:DATA_elab} for one of the experiments. Fig.~\ref{fig:distance_sensors} depicts the comparison between the three pre-processed distance measures with the ``ground truth'' from the motion tracker (left), and the DF based on the \emph{distance fusion} (right).

From Fig.~\ref{fig:distance_sensors} (left), it can be observed that RSU output is always available, while cameras generate signals only when RM$_\mathrm{c}$ is already near to the other RMs. When the output of the cameras is not available,  the \emph{distance fusion} is only computed based on the RSU. This is due to the computer vision system, which is unable to adequately detect the RM$_\mathrm{c}$ since it is confused with the laboratory background when it is far from cameras.

%*** Franca commenti qui per spiegare che quando c'è un solo segnale la fusione ovviamente riproduce il segnale, spiegare quindi che nei primi due secondo c'è solo il range sensor che è coperato dal risultato della fusion, spiegare che l'andamento a gradini è legato ad un oversampling che abbiamo fatto per allineare le misure che sono fatte da sensori che agiscono a frequenze diverse, dire ancora che WC e drone all'inizio non "vedono" l'ostacolo. ***

%From the above distance data, we c5n easily compute the speed and the acceleration *** Franca spiegare brevemente *** and then obtain the DF according to the procedure discussed in Sect.~\ref{sec:df}. 
Similar considerations can be done for the \emph{danger fusion}. The DF values computed by the three sensors are displayed and compared with the tracker data in Fig.~\ref{fig:dfs} (left). Those values are very noisy and unstable, while the fusion offers a smoother output that is more suitable to danger evaluation, as depicted by Fig.~\ref{fig:dfs} (right).

%This can be achieved at the sensor level, thus averaging the distance data in Fig.~\ref{fig:distance_sensors} or at the DF level, thus averaging the data in Fig.~\ref{fig:dfs} (left). The results of the two approached are displayed in Fig.~\ref{fig:dfs} (right). We call \emph{distance fusion} the first approach and \emph{danger fusion} the second.

For a quantitative evaluation, we computed a \emph{Root Mean Square Error} (RMSE) by comparing the DFs based on the tracker, with those obtained from the single sensors, and with the \emph{distance} and \emph{danger fusion} outputs. Such a descriptor cannot be computed for the \emph{voting fusion}, which returns a binary output. When coping with such outputs, we quantify the classification performance of the different methods in terms of accuracy, precision and recall. To interpret those measures, note that a \emph{false positive} is a case where a safe output is recognised as a dangerous situation. 
%In our over-cautious approach, we ideally want to reduce the number of \emph{false negatives}, corresponding to detecting the lack of danger for a dangerous scenario. 
The overall results are displayed in Tab.~\ref{tab:rmse}. 

%, that we want severely to avoid. 

In our experimentation with single technologies, the range sensors provided the best performance in terms of RMSE, accuracy, and precision. However, the AW camera obtained the best recall. %, although in a shorter time window. 
At the fusion level, the worst performance was given by the \emph{voting fusion}.
In spite of a higher RMSE compared to the \emph{danger fusion}, the accuracy of the 
\emph{distance fusion} was significantly higher. This confirms the idea that the best results are obtained by performing the fusion before any further signal processing \cite{hall}.

% \emph{Distance fusion} results to be the better case in terms of accuracy and precision as we actually expected in Subsec.~\ref{subsec:DATA_elab}.


\begin{figure}[htp!]  
\centering 
\begin{tikzpicture}[baseline,scale=0.7]
\pgfplotsset{xmin=0.5,xmax=4.2}
\begin{axis}[
legend style={at={(0.5,0.9)}},
axis y line*=left,ymin=0, ymax=3.5, xlabel=$t$ (s),
xtick={0.0,1.0,2.0,3.0,4.0},ylabel=danger $g$,ytick={1.0},yticklabels={$g^*$}]
\addplot[thick,color=orange,mark=none] table [smooth,x=timestamp,y=danger_range,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{range sensors}}
\addplot[thick,color=red,mark=none] table [smooth,x=timestamp,y=danger_wheelchair,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{AW camera}}
\addplot[thick,color=blue,mark=none] table [smooth,x=timestamp,y=danger_drone,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{drone camera}}
\addplot[very thick,dotted,color=black,mark=none] table [smooth,x=timestamp,y=danger_tracker,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{tracker}}
\draw[color=black!40,line width=0.25mm] (0,1) -- (5,1);
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}[baseline,scale=0.7]
\pgfplotsset{xmin=0.5,xmax=4.2}
\begin{axis}[legend style={at={(0.6,0.9)}},
axis y line*=left,ymin=0, ymax=3.5, xlabel=$t$ (s),
xtick={0.0,1.0,2.0,3.0,4.0},ytick={1.0},yticklabels={$g^*$}]
\addplot[very thick,color=black,mark=none] table [smooth,x=timestamp,y=danger_fusion,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{distance fusion}}
\addplot[very thick,color=black,dashed,mark=none] table [smooth,x=timestamp,y=danger_fusion_avg,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{danger fusion}}
\addplot[thick,dotted,color=black,mark=none] table [smooth,x=timestamp,y=danger_tracker,col sep=comma]{all.csv};
\addlegendentry{\scriptsize{tracker}}
\draw[color=black!40,line width=0.25mm] (0,1) -- (5,1);
\end{axis}
\end{tikzpicture}
\caption{DF computed from distances recorded by the sensors (left) and as obtained by \emph{danger} and \emph{distance fusion} (right).}
\label{fig:dfs}
\end{figure}

\begin{table}[htp]
\centering
\begin{tabular}{lp{1cm}rp{1cm}rrr}
\hline
Source/Fusion Technique&&RMSE&&Accuracy&Recall&Precision\\
\hline
Range sensors&&0.582&&{\bf 0.92}&0.89&{\bf 0.99}\\
AW camera&&0.948&&0.77&{\bf1.0}&0.59\\
Drone camera&&1.923&&0.51&0.63&0.32\\
\hline
Distance fusion&&0.447&&{\bf 0.92}&0.91&0.95\\
Danger fusion&&{\bf 0.361}&&0.83&0.78&0.96\\
Voting fusion&&-&&0.67&0.50&0.38\\
\hline
\end{tabular}
\caption{Performance evaluation of sensors and fusion techniques.}
\label{tab:rmse}
\end{table}



==> 08_Conclusions.tex <==
\section{Conclusions} \label{sec:conclusion}

In this paper, we have addressed the problem of safe road-crossing by autonomous wheelchairs supported by flying drones, using multi-sensor fusion. We have focused on the generation of a relevant laboratory dataset from multiple artificial vision and distance sensors installed on RoboMasters operating in ROS and OptiTrack enviroments. We made the dataset publicly available to the scientific community for further experimentation and performance evaluation. We also designed an analytical danger function to enable run-time risk assessment for road-crossing decision support. We have experimentally evaluated the danger function to provide some preliminary results as a proof-of-concept. The function is based on physical conditions and therefore represents a case of explainable decision fusion, whereas the output of some sensors, especially those based on artificial vision, is affected by a variable degree of opacity and uncertainty that need to be quantified to support probabilistic safety evaluation. Such an evaluation can be performed using an approach similar to the ones already introduced in  \cite{Flammini2020} and \cite{tas23}, and will be developed in future works. As future developments, we also plan to extend the dataset and experimentation with more complex real-world situations to be recognised and managed, such as multiple vehicles/obstacles from different directions, as well as with interference and disturbances due to vibrations, dirty camera lenses, glares, darkness, obstructions, weather conditions (rain, fog, etc.), some of which can be simulated by applying appropriate software filters. Although we focused on a specific application, we believe our contribution can be extended to other crossing scenarios, e.g., to support vision impaired people with similar assistive technologies.
